Numerical and asymptotic analysis of the three-dimensional electrohydrodynamic interactions of drop pairs

We study the pairwise interactions of drops in an applied uniform DC electric field within the framework of the leaky dielectric model. We develop three-dimensional numerical simulations using the boundary integral method and an analytical theory assuming small drop deformations. We apply the simulations and the theory to explore the electrohydrodynamic interactions between two identical drops with arbitrary orientation of the their line of centers relative to the applied field direction. Our results show complex dynamics depending on the conductivities and permittivities of the drops and suspending fluids, and the initial drop pair alignment with the applied electric field.

==> my_macros2.tex <==
\newcommand{\grbf}[1] {\mbox{\boldmath${#1}$\unboldmath}}
\newcommand{\al}{\alpha}
\newcommand{\kp}{\kappa}
%\newcommand{\tt}{\theta}
\newcommand{\Eb}{E_{\beta}}
\newcommand{\Tc}{\textsf{T}}
\newcommand{\altt}{\frac{\alpha}{\theta}}
\newcommand{\beq} {\begin{equation}}
\newcommand{\eeq} {\end{equation}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\bde}{\begin{description}}
\newcommand{\ede}{\end{description}}
\newcommand{\bce}{\begin{center}}
\newcommand{\ece}{\end{center}}
\newcommand{\ben} {\begin{enumerate}}
\newcommand{\een} {\end{enumerate}}
\newcommand{\bea} {\begin{eqnarray}}
\newcommand{\eea} {\end{eqnarray}}
\newcommand{\barr} {\begin{array}}
\newcommand{\earr} {\end{array}}
\newcommand{\bean} {\begin{eqnarray*}}
\newcommand{\eean} {\end{eqnarray*}}
% Change
\newcommand{\intg}[1]{\int_0^{2\pi} \int_0^\pi #1 \, du\, dv}
\newcommand{\pt}[1]{\frac{\partial #1}{\partial t}}
\newcommand{\iOm}[1]{\int_{\Omega(t)} #1 \, d\Omega}
\newcommand{\pn}[1]{\frac{\partial #1}{\partial n}}
\newcommand{\igt}[1]{\int_0^t\int_{\gamma(\tau)} #1 \,d\gamma dt}
\newcommand{\far}{\mathcal{S}_F}
\newcommand{\near}{\mathcal{S}_L}
%\renewcommand{\grbf}[1] {\mathbf{#1}}
\newcommand{\expt}[1] {e^{-n^2\pi^2({#1})}}
\newcommand{\gbf}[1] {\mathbf{#1}}
\newcommand{\dbl}{\mathcal{D}}
\newcommand{\sgl}{\mathcal{S}}
\newcommand{\mcd}{\mathcal{D}}
\newcommand{\mct}{\mathcal{T}}
\newcommand{\splf}{\phi_{\tilde{\sgl}}}
\newcommand{\bdp}{\rho}
\newcommand{\TODO}[1]{ \fbox{\parbox{3in}{\bf #1}}}
\newcommand{\ts}{\triangle t}
\newcommand{\phit}{\tilde{\phi}}
\newcommand{\phib}{\breve{\phi}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\sumn}{\sum_{n=1}^{p}}
\newcommand{\ifull}[1]{\int^{1}_{0} #1 \, d\theta}
\newcommand{\inear}[1]{\int^{10\alpha}_{0} #1 \, d\theta}
\newcommand{\ifar}[1]{\int_{10\alpha}^{1} #1 \, d\theta}
\newcommand{\ikers}[1]{\int_{0}^{1}\frac{1}{\theta^{\gamma}} #1 \, d\theta}
\newcommand{\ikerl}[1]{\int_{0}^{1}\log\theta #1 \, d\theta}
\newcommand{\kernel}{\frac{\sqrt{\alpha}} {\sqrt{\theta^3}} e^{-\frac{\alpha}{\theta}}}
\newcommand{\kernelJ}{\frac{1} {\sqrt{\theta}} e^{-\frac{\alpha}{\theta}}}
\newcommand{\bdry}[1]{\int_{\gamma} #1 \, d\gamma}
\newcommand{\bol}[1]{\textbf{#1}}
\newcommand{\sint}{S_n}
%\newcommand{\sintt}{S_{\textbf{n}}}
\newcommand{\sintt}[1]{\hat{#1}_{\mbk}}
\newcommand{\dsintt}{\tilde{S}_{n_1 n_2}}
\newcommand{\cost}{C_n}
\newcommand{\DG}{\frac{\partial G}{\partial n}}
\newcommand{\tick}{\textbf{{\small $\hookrightarrow $ resolved}}}

%% used in codes
\newcommand{\cellc}{c^c}
\newcommand{\radc}{r^c}
\newcommand{\sd}{\sqrt{\delta}}
\newcommand{\momc}{I_C}
\newcommand{\radg}{r^g}
\newcommand{\gausst}{G_{\delta}}
\newcommand{\rhat}{\mathbf{\hat{r}}}
\newcommand{\mbe}{\mathbf{E}}
\newcommand{\mbx}{\mathbf{x}}
\newcommand{\mby}{\mathbf{y}}
\newcommand{\mbxu}{|\mathbf{x}_u|}
\newcommand{\mbxa}{|\mathbf{x}_{\alpha}|}
\newcommand{\mbn}{\mathbf{n}}
\newcommand{\mbr}{\mathbf{r}}
\newcommand{\mbk}{\mathbf{k}}
\newcommand{\mck}{\mathcal{K}}
\newcommand{\mce}{\mathcal{E}}
\newcommand{\mcp}{\mathcal{P}}
\newcommand{\mcm}{\mathcal{M}}
\newcommand{\mcb}{\mathcal{B}}
\newcommand{\mbt}{{\mathbf t}}
\newcommand{\gauss}{\mathcal{G}}
\newcommand{\gaussD}{\mathcal{G}^D}
%\newcommand{\mbe}{\mathbf{e}}
\newcommand{\mbf}{\mathbf{f}}
\newcommand{\mbg}{\mathbf{g}}
\newcommand{\mbu}{\mathbf{u}}
\newcommand{\mba}{\mathbf{a}}
\newcommand{\mbb}{\mathbf{b}}
\newcommand{\cv}{\cos v}
\newcommand{\sv}{\sin v}
\newcommand{\lpb}{\triangle_S}
\newcommand{\norm}[1]{|\!| #1 |\!|}
\newcommand{\mbv}{\mathbf{v}}
\newcommand{\sdiv}{\text{div}_\gamma}
\newcommand{\Lg}{\mathcal{L}}
\newcommand{\sumy}{\sum_{n=0}^p \sum_{m=-n}^n}
\newcommand\defeq{\mathrel{\mathop :}=}
\newcommand{\vnm}{\mathbf{V}_n^m}
\newcommand{\wnm}{\mathbf{W}_n^m}
\newcommand{\jump}[1]{\left[\!\left[ #1 \right]\!\right]_{S^*}}

